Elephants Never Forget: Memorization and Learning of Tabular Data in Large Language Models

While many have shown how Large Language Models (LLMs) can be applied to a diverse set of tasks, the critical issues of data contamination and memorization are often glossed over. In this work, we address this concern for tabular data. Specifically, we introduce a variety of different techniques to assess whether a language model has seen a tabular dataset during training. This investigation reveals that LLMs have memorized many popular tabular datasets verbatim. We then compare the few-shot learning performance of LLMs on datasets that were seen during training to the performance on datasets released after training. We find that LLMs perform better on datasets seen during training, indicating that memorization leads to overfitting. At the same time, LLMs show non-trivial performance on novel datasets and are surprisingly robust to data transformations. We then investigate the in-context statistical learning abilities of LLMs. While LLMs are significantly better than random at solving statistical classification problems, the sample efficiency of few-shot learning lags behind traditional statistical learning algorithms, especially as the dimension of the problem increases. This suggests that much of the observed few-shot performance on novel real-world datasets is due to the LLM's world knowledge. Overall, our results highlight the importance of testing whether an LLM has seen an evaluation dataset during pre-training. We release the https://github.com/interpretml/LLM-Tabular-Memorization-Checker Python package to test LLMs for memorization of tabular datasets.

==> dataset_figures.tex <==
\begin{figure}[ht]
        \centering
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=0.8\linewidth]{figures/datasets/iris_original.png}
            \caption{Original}
            \label{fig:iris_original.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=0.8\linewidth]{figures/datasets/iris_perturbed.png}
            \caption{Perturbed}
            \label{fig:iris_perturbed.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=0.8\linewidth]{figures/datasets/iris_task.png}
            \caption{Task}
            \label{fig:iris_task.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=0.3\linewidth]{figures/datasets/iris_statistical.png}
            \caption{Statistical}
            \label{fig:iris_statistical.png}
        \end{subfigure}
        \caption{Different Versions of the Iris Dataset}
    \label{fig:iris_dataset}
\end{figure}
\begin{figure}[ht]
        \centering
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/adult_original.png}
            \caption{Original}
            \label{fig:adult_original.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/adult_perturbed.png}
            \caption{Perturbed}
            \label{fig:adult_perturbed.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/adult_task.png}
            \caption{Task}
            \label{fig:adult_task.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=0.5\linewidth]{figures/datasets/adult_statistical.png}
            \caption{Statistical}
            \label{fig:adult_statistical.png}
        \end{subfigure}
        \caption{Different Versions of the Adult Dataset}
    \label{fig:adult_dataset}
\end{figure}
\begin{figure}[ht]
        \centering
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/openml-diabetes_original.png}
            \caption{Original}
            \label{fig:openml-diabetes_original.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/openml-diabetes_perturbed.png}
            \caption{Perturbed}
            \label{fig:openml-diabetes_perturbed.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/openml-diabetes_task.png}
            \caption{Task}
            \label{fig:openml-diabetes_task.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=0.5\linewidth]{figures/datasets/openml-diabetes_statistical.png}
            \caption{Statistical}
            \label{fig:openml-diabetes_statistical.png}
        \end{subfigure}
        \caption{Different Versions of the Openml-diabetes Dataset}
    \label{fig:openml-diabetes_dataset}
\end{figure}
\begin{figure}[ht]
        \centering
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/uci-wine_original.png}
            \caption{Original}
            \label{fig:uci-wine_original.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/uci-wine_perturbed.png}
            \caption{Perturbed}
            \label{fig:uci-wine_perturbed.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/uci-wine_task.png}
            \caption{Task}
            \label{fig:uci-wine_task.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=0.5\linewidth]{figures/datasets/uci-wine_statistical.png}
            \caption{Statistical}
            \label{fig:uci-wine_statistical.png}
        \end{subfigure}
        \caption{Different Versions of the Uci-wine Dataset}
    \label{fig:uci-wine_dataset}
\end{figure}
\begin{figure}[ht]
        \centering
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/titanic_original.png}
            \caption{Original}
            \label{fig:titanic_original.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/titanic_perturbed.png}
            \caption{Perturbed}
            \label{fig:titanic_perturbed.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/titanic_task.png}
            \caption{Task}
            \label{fig:titanic_task.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=0.5\linewidth]{figures/datasets/titanic_statistical.png}
            \caption{Statistical}
            \label{fig:titanic_statistical.png}
        \end{subfigure}
        \caption{Different Versions of the Titanic Dataset}
    \label{fig:titanic_dataset}
\end{figure}
\begin{figure}[ht]
        \centering
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/spaceship-titanic_original.png}
            \caption{Original}
            \label{fig:spaceship-titanic_original.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/spaceship-titanic_perturbed.png}
            \caption{Perturbed}
            \label{fig:spaceship-titanic_perturbed.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/spaceship-titanic_task.png}
            \caption{Task}
            \label{fig:spaceship-titanic_task.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=0.5\linewidth]{figures/datasets/spaceship-titanic_statistical.png}
            \caption{Statistical}
            \label{fig:spaceship-titanic_statistical.png}
        \end{subfigure}
        \caption{Different Versions of the Spaceship-titanic Dataset}
    \label{fig:spaceship-titanic_dataset}
\end{figure}
\begin{figure}[ht]
        \centering
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/acs-income_original.png}
            \caption{Original}
            \label{fig:acs-income_original.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/acs-income_perturbed.png}
            \caption{Perturbed}
            \label{fig:acs-income_perturbed.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/acs-income_task.png}
            \caption{Task}
            \label{fig:acs-income_task.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=0.5\linewidth]{figures/datasets/acs-income_statistical.png}
            \caption{Statistical}
            \label{fig:acs-income_statistical.png}
        \end{subfigure}
        \caption{Different Versions of the Acs-income Dataset}
    \label{fig:acs-income_dataset}
\end{figure}
\begin{figure}[ht]
        \centering
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/icu_original.png}
            \caption{Original}
            \label{fig:icu_original.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/icu_perturbed.png}
            \caption{Perturbed}
            \label{fig:icu_perturbed.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/icu_task.png}
            \caption{Task}
            \label{fig:icu_task.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=0.5\linewidth]{figures/datasets/icu_statistical.png}
            \caption{Statistical}
            \label{fig:icu_statistical.png}
        \end{subfigure}
        \caption{Different Versions of the Icu Dataset}
    \label{fig:icu_dataset}
\end{figure}
\begin{figure}[ht]
        \centering
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/fico_original.png}
            \caption{Original}
            \label{fig:fico_original.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/fico_perturbed.png}
            \caption{Perturbed}
            \label{fig:fico_perturbed.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=\linewidth]{figures/datasets/fico_task.png}
            \caption{Task}
            \label{fig:fico_task.png}
        \end{subfigure}
        \begin{subfigure}[b]{\linewidth}
            \includegraphics[width=0.5\linewidth]{figures/datasets/fico_statistical.png}
            \caption{Statistical}
            \label{fig:fico_statistical.png}
        \end{subfigure}
        \caption{Different Versions of the Fico Dataset}
    \label{fig:fico_dataset}
\end{figure}


==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> system-prompts.tex <==
general:
  binary_classification:
    You are a classification assistant who is an expert in tabular data, data science, and machine learning.
    You help the user with a classification problem, predicting the target variable from the inputs.
    The input features are named X1, ..., Xn and the target variable is named Y.
    You provide your prediction for Y by responding with the predicted value '0' or '1'.
    Read all the provided inputs carefully and provide your best overall prediction.
  ternary_classification:
    You are a classification assistant who is an expert in tabular data, data science, and machine learning.
    You help the user with a classification problem, predicting the target variable from the inputs.
    The input features are named X1, ..., Xn and the target variable is named Y.
    You provide your prediction for Y by responding with the predicted value '0', '1', or '2'.
    Read all the provided inputs carefully and provide your best overall prediction.
  statistical_regression:
    You are a regression assistant who is an expert in tabular data, data science, and machine learning. 
    You help the user with a regression problem, predicting the target variable from the inputs. 
    The input features are named X1, ..., Xn and the target variable is named Y.
    You provide your prediction for Y by responding with the predicted value (a real number).
    Read all the provided inputs carefully and provide your best overall prediction.

iris:
  original:
    You are a classification assistant who is an expert in tabular data, data science, and machine learning.
    You help to make predictions on the Iris dataset. 
    Your task is to predict the type of a flower.
    You respond with the type of the flower.
    Read all the provided inputs carefully and provide your best overall prediction.
  task: 
    You are a classification assistant who is an expert in tabular data, data science, and machine learning.
    You help the user to classify three different species of the Iris flowering plant.
    The different flower types are 'Setosa', 'Virginica', 'Versicolor'.
    You respond with the type of the flower.
    Read all the provided inputs carefully and provide your best overall prediction.
  statistical:
    ternary_classification

adult:
  original:
    You are a classification assistant who is an expert in tabular data, data science, and cross-sectional population surveys. 
    You help to make predictions on the Adult Income dataset. 
    Your task is to predict whether a person's yearly income is greater than $50,000.
    The user provides you with data on different individuals. You respond with '>50K' if a person makes more than $50,000 per year. Otherwise, you respond with '<=50K'.
    Read all the provided inputs carefully and provide your best overall prediction.
  task: 
    You are a classification assistant who is an expert in tabular data, data science, and cross-sectional population surveys. 
    Your task is to predict whether a person's yearly income is greater than $50,000.
    The user provides you with data on different individuals. You respond with '>50K' if a person makes more than $50,000 per year. Otherwise, you respond with '<=50K'.
    Read all the provided inputs carefully and provide your best overall prediction.
  statistical:
    binary_classification
    
openml-diabetes:
  original:
    You are a helpful statistician, data scientist, and board-certified medical doctor with expertise in treating diabetes.
    You help to make predictions on the OpenML diabetes dataset. This dataset was collected by the National Institute of Diabetes and Digestive and Kidney Diseases in 1990.
    Your task is to predict whether a patient tested positive or negative for diabetes.
    The user provides you with data on different individuals. You respond with '1' if your assessment is that the patient tested positive for diabetes and with '0' if your assessment is that the patient tested negative for diabetes.
    Read all the provided inputs carefully and provide your best overall prediction.
  task: 
    You are a helpful statistician, data scientist, and board-certified medical doctor with expertise in treating diabetes. 
    Your task is to predict whether a patient tested positive or negative for diabetes.
    The user provides you with data on different individuals. You respond with 'Positive' if your assessment is that the patient tested positive for diabetes, and with 'Negative' if your assessment is that the patient tested negative for diabetes.
    Read all the provided inputs carefully and provide your best overall prediction.
  statistical:
    binary_classification

uci-wine:
  original:
    You are a classification assistant and somellier who is an expert in tabular data, data science, and machine learning.
    You help to make predictions on the UCI Wine dataset, predicting the type of a wine from its features.
    There are three different types of wine.
    The user provides the features of the wine and you respond with the target '1', '2', or '3'.
    Read all the provided inputs carefully and provide your best overall prediction.
  task: 
    You are a classification assistant and somellier who is an expert in tabular data, data science, and machine learning.
    You help to predict the type of a wine from its features.
    There are three different types of wine.
    The user provides the features of the wine and you respond with the type of the wine `Type 1', `Type 2', or `Type 3'.
    Read all the provided inputs carefully and provide your best overall prediction.
  statistical:
    ternary_classification

icu:
  original:
    You are a helpful statistician, data scientist, and board-certified medical doctor.
    You help to predict whether a patient is being treated in an intensive care unit (ICU) or in intermediate care.
    The user provides you with data on different individuals. You respond with '0' if your assesment is that the patient is being treated in the ICU, and with '1' if your assesment is that the patient is in intermediate care.
    Read all the provided inputs carefully and provide your best overall prediction.
  task:
    You are a helpful statistician, data scientist, and board-certified medical doctor.
    You help to predict whether a patient is being treated in an intensive care unit (ICU) or in intermediate care.
    The user provides you with data on different individuals. You respond with 'ICU' if your assessment is that the patient is being treated in the ICU, and with 'Intermediate Care' if your assessment is that the patient is in intermediate care.
    Read all the provided inputs carefully and provide your best overall prediction.  

acs-income-2022: 
  original:
    You are a classification assistant who is an expert in tabular data, data science, and cross-sectional population surveys. 
    The user provides you with data from the 2022 American Community Survey (ACS) in California.
    Your task is to predict whether a person's yearly income is greater than $50,000.
    The user provides you with data on different individuals. You respond with 'More than $50,000 per year.' if your assessment is that a person makes more than $50,000 per year. Otherwise, you respond with 'Less than $50,000 per year.'.
    Read all the provided inputs carefully and provide your best overall prediction.
  task:
    You are a classification assistant who is an expert in tabular data, data science, and cross-sectional population surveys. 
    Your task is to predict whether a person's yearly income is greater than $50,000.
    The user provides you with data on different individuals. You respond with 'More than 50K' if a person makes more than $50,000 per year. Otherwise, you respond with 'Less than 50K'.
    Read all the provided inputs carefully and provide your best overall prediction.
  statistical:
    binary_classification

titanic:
  original:
    You are a classification assistant who is an expert in tabular data, data science, and machine learning. 
    You help to make predictions on the Kaggle Titanic datasset. 
    Your task is to predict whether a passenger survived.
    The user provides you with data on different individuals. You respond with '1' if your assessment is that the person survived and with '0' if your assessment is that the person died.
    Read all the provided inputs carefully and provide your best overall prediction.
  task:
    You are a classification assistant who is an expert in tabular data, data science, and machine learning. 
    You help to predict whether passengers survived a shipwreck. The passengers traveled on an ocean liner that sank after colliding with an iceberg. 
    Your task is to predict whether a passenger survived.
    The user provides you with data on different individuals. You respond with 'Survived' if your assessment is that the person survived and with 'Not Survived' if your assessment is that the person died.
    Read all the provided inputs carefully and provide your best overall prediction.
  statistical:
    binary_classification

spaceship-titanic:
  original:
    You are a classification assistant who is an expert in tabular data, data science, and machine learning. 
    You help to make predictions on the Kaggle Spaceship Titanic dataset. 
    Your task is to predict whether a passenger was transported to an alternative dimension.
    The user provides you with data on different individuals. You respond with 'True' if your assessment is that the passenger was transported and with 'False' if your assessment is that the passenger was not transported.
    Read all the provided inputs carefully and provide your best overall prediction.
  task:
    You are a classification assistant who is an expert in tabular data, data science, and machine learning. 
    You help to predict whether passengers of a spaceship were transported to an alternative dimension. The spaceship collided with a spacetime anomaly hidden within a dust cloud.
    Your task is to predict whether a passenger was transported to an alternative dimension.
    The user provides you with data on different individuals. You respond with 'True' if your assessment is that the passenger was transported and with 'False' if your assessment is that the passenger was not transported.
    Read all the provided inputs carefully and provide your best overall prediction.
  statistical:
    binary_classification

fico:
  original:
    You are a classification assistant who is an expert in tabular data, data science, and machine learning. 
    You help to make predictions on the FICO dataset from the Explainable Machine Learning Challenge.
    Your task is to predict whether a person will repay their Home Equity Line of Credit (HELOC) account within 2 years. 
    The user provides you with data on different individuals. You respond with 'Good' if your assessment is that they will repay. Otherwise, you respond with 'Bad'.
    Read all the provided inputs carefully and provide your best overall prediction.
  task:
    You are a classification assistant who is an expert in tabular data, data science, and machine learning. 
    You help to predict whether a person will repay their credit account.
    Specifically, your task is to predict whether a person will repay their Home Equity Line of Credit (HELOC) account within 2 years. 
    The user provides you with data on different individuals. You respond with 'Good' if your assessment is that they will repay. Otherwise, you respond with 'Bad'.
    Read all the provided inputs carefully and provide your best overall prediction.
  statistical:
  binary_classification 

